An Efficient Real-Time NMPC for Quadrotor Position Control under Communication Time-Delay

The advances in computer processor technology have enabled the application of nonlinear model predictive control (NMPC) to agile systems, such as quadrotors. These systems are characterized by their underactuation, nonlinearities, bounded inputs, and time-delays. Classical control solutions fall short in overcoming these difficulties and fully exploiting the capabilities offered by such platforms. This paper presents the design and implementation of an efficient position controller for quadrotors based on real-time NMPC with time-delay compensation and bounds enforcement on the actuators. To deal with the limited computational resources onboard, an offboard control architecture is proposed. It is implemented using the high-performance software package acados, which solves optimal control problems and implements a real-time iteration (RTI) variant of a sequential quadratic programming (SQP) scheme with Gauss-Newton Hessian approximation. The quadratic subproblems (QP) in the SQP scheme are solved with HPIPM, an interior-point method solver, built on top of the linear algebra library BLASFEO, finely tuned for multiple CPU architectures. Solution times are further reduced by reformulating the QPs using the efficient partial condensing algorithm implemented in HPIPM. We demonstrate the capabilities of our architecture using the Crazyflie 2.1 nano-quadrotor.

==> content/control_architecture.tex <==
\label{sec:control_arch}
Given the constraints regarding the resources available on the UAV, in terms of both computational and self-sensing capabilities, part of the control task needs to be executed on a hardware physically disconnected to the UAV. Thus, one can distinguish the onboard from the offboard control tasks. 

%Knowing the large delay concerning the radio communication (see \cite{dubois2018,fernando}) and the different characteristic times of different part of the system dynamics a hierarchical control architecture has been chosen. In this framework we can mainly distinguish two level, the high-level control tasks and the low-level one, as a general rule the the output of the high level computation serve as input for the low level part.

All the on-board tasks are low-level tasks.

The on-board control tasks consist of all the computations happening
on the electronic components attached to the UAV which are not considered part of the plant,
those tasks can be dived further in the following set: radio subsystem, attitude controller, rate controller and motor mixer.

The off-board control computation motion capture high level.

As shown in Figure \ref{fig:block_diagram} the signals sent between the off-board controller (NMPC)
and on-board  

Low level controller needed to stabilize fast dynamics
limited computation resource on board
big delay off-board

As shown in Figure \ref{fig:block_diagram} several abstractions are build on top
the environment in which the locomotion problem in this study lives.


We first distinguish from the on board

e call plant physical system with the following interfaces with the digital abstraction of the controller:
* Four PWM signals for motor driver
* IMU and gyroscope signals
* Brightness on the pixel of the camera of the Mocap



==> content/low_level.tex <==
The way in which the high-level controller (NMPC) setpoints are used by the faster feedback loops (PIDs) in our hierarchical control architecture is not entirely conventional and deserves some considerations.

Two main points presented in Fig. \ref{fig:block_diagram} should be addressed: first, the control input considered in the formulation of the NMPC does not correspond to the reference signal tracked by the PID loops entirely. Instead, part of predicted state $\xi^{*}(t)$ is used together with the aforementioned optimal control inputs $u^{*}(t)$ to reconstruct the real standard input commands passed as setpoint to the Crazyflie.  Second, part of the control input is sent as setpoint to the outer control loop (Attitude Controller) and another part is sent to the inner loop (Rate Controller) instead. Furthermore, as mentioned in Section \ref{subsec:nmpc}, the PID loops are not included in the model used in the NMPC formulation, meaning that this model does not represent truly the real system, not even in the case of perfect knowledge of the physical parameters. As a consequence, the feedback policy predicted in the optimal solution is distorted in the real system by the PID. Notice that, intuitively by reducing the time of the NMPC discretization, the distortion can be mitigated. Thus, one possible solution is to implement a linear interpolation onboard, considering the frequency of each loop, that, given a new desired command input from the NMPC, constructs data points that are passed as reference signals to the PIDs.



==> content/nmpc_time_delay.tex <==
\label{sec:nmpc}

==> content/pid_controller.tex <==
The first considered controller is a PID acting separately on each axis of $\{\mathcal{B}\}$.
